Closed-loop Analysis of Vision-based Autonomous Systems: A Case Study

Deep neural networks (DNNs) are increasingly used in safety-critical autonomous systems as perception components processing high-dimensional image data. Formal analysis of these systems is particularly challenging due to the complexity of the perception DNNs, the sensors (cameras), and the environment conditions. We present a case study applying formal probabilistic analysis techniques to an experimental autonomous system that guides airplanes on taxiways using a perception DNN. We address the above challenges by replacing the camera and the network with a compact probabilistic abstraction built from the confusion matrices computed for the DNN on a representative image data set. We also show how to leverage local, DNN-specific analyses as run-time guards to increase the safety of the overall system. Our findings are applicable to other autonomous systems that use complex DNNs for perception.

==> section_eval_old.tex <==
\section{Experiments}
\label{sec:eval}
%In this section we report on experiments demonstrating probabilistic safety analysis for the two case studies, center-line tracking and line-following robot.
In this section we report on experiments demonstrating probabilistic safety analysis for the case study of center-line tracking.

%For TaxiNet our industry partner developed a CNN model with 24 layers; input layer taking in 360 × 200 × 3 images, 5 convolution layers, and four dense layers (100/50/10 ELU neurons) before the output layer. The model was trained and tested using images generated by the X-Plane simulator [CITE] and the Mean Absolute Error (MAE) on test set is 0.366 for $\vcte$ and 1.645 for he respectively. 
%The complex architecture of the model, specifically the ELU activation function, impedes the application of existing DNN verification tools (such as ~\cite{KatzHIJLLSTWZDK19}). Further, we do not have access to the training dataset for the model. This scenario is representative of realistic applications wherein complex pre-trained models are employed. In this work, we leverage rules abstracting input-output behavior of the model to act as probabilistic verification conditions for closed-loop analysis, thereby demonstrating the application of our safety analysis in a realistic setting. However, in order to also demonstrate the effect of some popular run-time checks such as robustness and confidence calibration [CITE], we build a simpler classifier model for the line-following robot problem. It has the same dynamics as the autonomous taxiing system but where the sensor readings are simpler images generated using the Gazebo simulator. These two case-studies highlight the benefit of our analysis framework, which enables plugging in DNNs of different sizes, complexity and verification techniques specific to the underlying models.

%Our industry partner developed a CNN model for TaxiNet with 24 layers; input layer taking in 360 × 200 × 3 images, 5 convolution layers, and four dense layers (100/50/10 ELU neurons) before the output layer. %The model was trained and tested using images generated by the X-Plane simulator [CITE] and the Mean Absolute Error (MAE) on test set is 0.366 for $\vcte$ and 1.645 for $\vhe$ respectively. 
%The complex architecture of the model, specifically the ELU activation function, impedes the application of existing verification techniques (such as ~\cite{KatzHIJLLSTWZDK19}). Further, we do not have access to the training dataset for the model.  This scenario is representative of realistic applications wherein complex pre-trained models are employed. In this work, we leverage rules abstracting input-output behavior of the model to act as probabilistic verification conditions, thereby demonstrating the application of our safety analysis in a realistic setting. %However, in order to also demonstrate the effect of some popular run-time checks such as robustness and confidence calibration [CITE], we build a simpler classifier model for the line-following robot problem. It has the same dynamics as the autonomous taxiing system but where the sensor readings are simpler images generated using the Gazebo simulator. These two case-studies highlight the benefit of our analysis framework, which enables plugging in DNNs of different sizes, complexity and verification techniques specific to the underlying models.

%-Demonstrate that actual performance coincides with verification results\\

\subsection{Center-line Tracking using TaxiNet}
\label{sec:eval_taxinet}
%The TaxiNet model from our industry partner was trained and tested using images generated by the X-Plane simulator~\cite{xplane}. 
The TaxiNet perception model from our industry partner is a regression CNN with  24 layers; input layer taking in 360 × 200 × 3 images, 5 convolution layers, and four dense layers (100/50/10 ELU neurons) before the output layer. 
We used a representative data set with 11108 images, provided by the industry partner (including images with different environment conditions such as shadow, skid marks, intersections and night-time).  
The model has a Mean Absolute Error (MAE)  of  1.185 for $\vcte$ and 7.86 for $\vhe$ outputs respectively. The closed-loop system encoded as a DTMC is shown in the Appendix~\ref{sec:dtmc_prism}.
%with deterministic modules for the controller and vehicle dynamics, and a probabilistic automaton encoding the transition probabilities of the Boeing model.

%\paragraph{Transition Probabilities Calculation:}
We discretized the $\vcte$ output into three bins (i.e., labels) as follows:
\begin{itemize}
\item class "1" (\emph{left} of center-line): -8.0 meters $<=$ $\vcte$ $<=$ -2.67 meters, 
\item class "0" (\emph{on} center-line): -2.67 meters $<$ $\vcte$ $<=$ 2.66 meters, 
\item class "2" (\emph{right} of center-line): 2.66 meters $<$ $\vcte$ $<=$ 8.0 meters.
\end{itemize}

The $\vhe$ output is discretized as follows: 

\begin{itemize}
\item label "1" (\emph{heading left}): -35.0 degrees $<=$ $\vhe$ $<=$ -11.67 degrees, 
\item label "0" (\emph{heading straight}): -11.67 degrees $<$ $\vhe$ $<=$ 11.66 degrees, 
\item label "2" (\emph{heading right}): 11.66 degrees $<$ $\vhe$ $<=$ 35.0 degrees.
\end{itemize}

We also experimented with finer discretization of the $\vcte$ output into five bins as follows:
\begin{itemize}
\item class "3" (\emph{far left} of center-line): -8.0 meters $<=$ $\vcte$ $<=$ -4.8 meters,
\item class "1" (\emph{left} of center-line): -4.8 meters $<=$ $\vcte$ $<=$ -1.6 meters, 
\item class "0" (\emph{on} center-line): -1.6 meters $<$ $\vcte$ $<=$ 1.6 meters, 
\item class "2" (\emph{right} of center-line): 1.6 meters $<$ $\vcte$ $<=$ 4.8 meters,
\item class "4" (\emph{far right} of center-line): 4.8 meters $<=$ $\vcte$ $<=$ 8.0 meters.
\end{itemize}
The classification accuracy of the discretized models on the test dataset were as follows; 3-bin: 78.67\% for $\vcte$, 69.99\% for $\vhe$, 5-bin: 62.39\% for $\vcte$, 69.99\% for $\vhe$.
%For every label, we calculated the probabilities for correct classification to the respective label and mis-classification to each of the other labels. 
The confusion matrices (computed on the representative dataset) and the corresponding transition probabilities are shown in Tables ~\ref{tab:trans_prob},~\ref{tab:trans_prob_5}  in the Appendix ~\ref{sec:tables}.  

\divya{to be updated based on 5-bin table} The discretized view of the network already provides some useful insights.
%regarding its behavior in terms of the discrete states relevant to the closed-loop analysis. 
For instance the model performs best for inputs lying on the center-line; this can be attributed to the fact that the model was trained mainly on scenarios where the plane follows the center-line. Note also that the model is of good quality, as it does not misclassify inputs on the \emph{left} as being on the \emph{right} and vice-versa (0 observations for 1-2 and 2-1 in Table~\ref{tab:trans_prob}).  To confirm the lack of misclassification in such cases one would need  a {\em proof} which we leave for future work.
%wrt. the $\vcte$ output and inputs \emph{heading left} wrt. the $\vhe$ output. The training of the model has been focused on scenarios where the plane is \emph{on} the center-line. This uneven distribution of inputs across the bins (also reflected in our dataset refer Table~\ref{tab:trans_prob}) impacts model behavior. The model mis-classifies the $\vcte$ output for inputs lying on either side of the center (specifically \emph{left}) as being \emph{on} the center-line. However, one can observe that there are no mis-classifications of inputs on the \emph{left} as being on the \emph{right} and vice-versa (0 transitions for 1-2 and 2-1 in Table~\ref{tab:trans_prob}). Formal proofs for such transitions can provide guarantees of robustness of the model in these cases. 
It is also interesting to note that the behavior wrt. the $\vhe$ prediction could be attributed to the position of the camera which is on the right wing of the plane; the nose and center-line are most visible when heading left and are occluded when heading right. %Such observations can inform better setup for training of the model. 
A more precise analysis of the model behavior can be obtained by having a finer discretization %(including labels such as\emph{far left}, and \emph{far right} of center-line, and more heading directions), 
and more inputs for each bin.
%\divya{do we need to mention about 1-2 and 2-1 have 0 transitions and the idea to prove them to get guarantees?}
%\corina{yes} \divya{I have tried to incorporate this in the paragraph above, But perhaps we should include this in 4.3 or in future work , since we can not do any proofs on the Boeing model.}

%\corina{{\bf Todo:} say we can refine the discretization by considering more bins/labels.}\divya{I have mentioned this in the last sentence of the previous paragraph. What else could we add?}

%\corina{ also comment a bit on the table: the results already indicate that some situations require more data; } \divya{I have mentioned " The uneven distribution of inputs across the bins (refer Table~\ref{tab:trans_prob}) can also impact the behavior". Should I elaborate?}

%\corina{also that the neural network tends to make more mistakes when the airplane is on the right of the center line; this may be due to the camera positioning on the left hand side?}\divya{ The current results indicate that the model makes more mistakes for $\vcte$ prediction when the plane is on the LEFT side of the center-line, and more mistakes for $\vhe$ prediction when the plane is on the RIGHT side. I have explained this in the paragraph above with possible reasons}.

\paragraph{Mining Rules for Run-time Guards.} 
%The complex architecture of the model, specifically the ELU activation function, impedes the application of existing verification approaches (such as ~\cite{HuangKWW16,abs-1710-00486,GuoPSW17,KatzHIJLLSTWZDK19}) to the model. Furthermore, we do not have access to the training dataset for the model.  In this work, we leverage rules abstracting input-output behavior of the model to act as probabilistic verification conditions, thereby demonstrating the application of our safety analysis in a realistic setting.
The complex architecture of the Boeing Taxinet model impedes the application of existing verification approaches for DNNs processing images, which have typically been applied to classifier models[CITE], or to simple regression models[CITE]. 

Previous work ~\cite{KadronGPY21} has explored the use of rules mined from the TaxiNet model for the purpose of explaining correct and incorrect model behavior. The rules are in the form of $Pre \implies Post$, where the $Pre$ condition is in terms of neuron constraints in the latent space of the network and characterizes inputs on which the $Post$ condition (property of the network outputs) is satisfied~\cite{ASE19}. The following correctness property of the regression outputs was considered in~\cite{KadronGPY21}, $|\vcte_{est}-\vcte| \leq 1.0~\mathit{meters} \; \wedge \; |\vhe_{est}-\vhe| \leq 5~ \mathit{degrees}$, and rules for the satisfaction and violation of this property were extracted. 

Leveraging this work, we extracted rules for valid and invalid behavior at each of the 3 dense layers of the model using a separate set of 5554 test inputs. 
Example of a rule for invalid behavior: 
$N_{1,85} <= -0.998 \wedge N_{2,50} <= 3.31 \wedge N_{1,84} <= -0.994 \wedge N_{1,15} > -0.999 \wedge$$
$$ N_{1,21} <= 1.711 \wedge N_{1,70} <= 11.088 \wedge N_{1,51} > -0.999 \wedge N_{1,21} > -0.637 \implies |\vcte_{est}-\vcte| > 1.0~\mathit{meters} \; \lor \; |\vhe_{est}-\vhe| > 5~\mathit{degrees}$.
Here $N_{i,j}$ indicates the $j^{th}$ neuron in the $i^{th}$ dense layer. This rule has a support of 755 , indicating that 755 (out of 5554) inputs satisfied the neuron pattern and the DNN violated the safety property for each of them.% The validation precision and recall of the rule is 97.79\% and 2\% respectively. 

For our case study, we experimented with deploying the rules for invalid behavior as run-time guards to catch inputs potentially leading to misbehavior. %In order to obtain good coverage while maintaining high precision, 
We selected the top two rules with the highest support from each layer and deployed them as run-time guards. When running on the dataset with 11108 inputs, inputs that satisfied any of the selected rules were discarded (1983 inputs), thereby abstaining the model from potential misbehavior. 
%The regression model behavior improved (MAE for $\vcte$: 1.07, MAE for $\vhe$: 6.39), which in turn improved the accuracies on the classification abstraction as well ($\vcte$: 78.82\%, $\vhe$:76\%). 
The new confusion matrix (computed for the inputs that pass the run-time guard) and transition probabilities are shown in Table~\ref{tab:trans_prob_vc} in the Appendix ~\ref{sec:tables}. Note that we could easily deploy other run-time guards using e.g., the rules for valid behavior, or rules for correct/incorrect behavior wrt. the discretized outputs. 
The resulting transition probabilities can be easily integrated into the existing DTMC model. 
\corina{We chose the rules for invalid behavior because...}

\paragraph{Results for \prism{} Analysis.}
The \prism{} code corresponding to the two DTMC models, $M_1$ and $M_2$ (denoting the closed-loop system without and with run-time guard respectively), are shown in the Appendix~\ref{sec:dtmc_prism}. The scenario considered was the airplane moving forward in a straight line for a fixed number of steps. The system was analyzed to compute the probability of failure in violating the two safety properties encoded in PCTL; {\em Property 1:} $P=? [ F (\vcte=-1)]$, and {\em Property 2:}
$P=? [ F (\vhe=-1)]$.

The results for running \prism{} on the two models on the two safety properties are shown in Figures~\ref{fig:prism_results_3bins} and \ref{fig:prism_results_5bins}; where $N$ is the number of steps in DTMC. The results highlight the benefit of the run-time guard. %Running \prism{} is virtually instantaneous.

\begin{figure*}[]
    \centering
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[height=2.0in]{taxinet_plots/prism/taxinet_3bin_p1_30.png}
        \caption{The probability of $\vcte$ failure ($P=? [ F (\vcte=-1)]$)}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[height=2.0in]{taxinet_plots/prism/taxinet_3bin_p2_30.png}
        \caption{The probability of $\vhe$ failure ($P=? [ F (\vhe=-1)]$)}
    \end{subfigure}%
    \\
    % \begin{subfigure}[t]{0.475\textwidth}
    %     \centering
    %     \includegraphics[height=2.0in]{taxinet_plots/taxinet_conditional.pdf}
    %     \caption{The probability of $\vcte$ or $\vhe$ failure given the input passes the run-time guard ($P=? [ F (\vcte=-1 \vee \vhe=-1) \mid G(v=1)]$)}
    % \end{subfigure}%  
    %~
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[height=2.0in]{taxinet_plots/prism/taxinet_3bin_p3_30.png}
        \caption{The probability of abort due to run-time guard failure ($P=? [ F (v=0~\&~i=M)]$)}
    \end{subfigure}%   
    \caption{Probabilistic model checking results for 3-bins model via \prism{} \label{fig:prism_results_3bins}}
\end{figure*}

\begin{figure*}[]
    \centering
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[height=2.0in]{taxinet_plots/prism/taxinet_5bin_p1_30.png}
        \caption{The probability of $\vcte$ failure ($P=? [ F (\vcte=-1)]$)}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[height=2.0in]{taxinet_plots/prism/taxinet_5bin_p2_30.png}
        \caption{The probability of $\vhe$ failure ($P=? [ F (\vhe=-1)]$)}
    \end{subfigure}%
    \\
    % \begin{subfigure}[t]{0.475\textwidth}
    %     \centering
    %     \includegraphics[height=2.0in]{taxinet_plots/taxinet_conditional.pdf}
    %     \caption{The probability of $\vcte$ or $\vhe$ failure given the input passes the run-time guard ($P=? [ F (\vcte=-1 \vee \vhe=-1) \mid G(v=1)]$)}
    % \end{subfigure}%  
    %~
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[height=2.0in]{taxinet_plots/prism/taxinet_5bin_p3_30.png}
        \caption{The probability of abort due to run-time guard failure ($P=? [ F (v=0~\&~i=M)]$)}
    \end{subfigure}%   
    \caption{Probabilistic model checking results for 5-bins model via \prism{} \label{fig:prism_results_5bins}}
\end{figure*}

%\begin{table}[ht!]
%    \centering
    %\caption{Results for \prism{} Analysis (to be replaced with a graph)}
   
%    \begin{tabular}{c|c|c|c||c|c|c|}
%    \multicolumn{1}{c}{}&\multicolumn{3}{c}{Property 1}&\multicolumn{3}{c}{Property 2}\\
%    \cline{2-7}
%    N& $M_1$ & $M_2$ & $M_3$ & $M_1$ & $M_2$ & $M_3$ \\
%    \cline{2-7}
    %3&  & & & \\
    %4&  & & & \\
%    10& 0.391 & 0.208 & 0.302 & 0.060 & 0.290 & 0.027\\
%    20& 0.632 & 0.335 & 0.538 & 0.099 & 0.465 & 0.049\\
%    30& 0.749 & 0.385 & 0.683 & 0.118 & 0.535 & 0.063\\
%    \cline{2-7}
%    \end{tabular}
%    \caption{\prism{} Results for Properties 1 \& 2 (3 bins); $M_1$: without run-time guard; $M_2$: with run-time guard; $M_3$: with run-time guard hard-coded to always pass}
    %\label{tab:prism_results}
%\end{table}

%\begin{table}[ht!]
%    \centering
%    %\caption{Results for \prism{} Analysis (to be replaced with a graph)}
   
%    \begin{tabular}{c|c|c|c||c|c|c|}
%    \multicolumn{1}{c}{}&\multicolumn{3}{c}{Property 1}&\multicolumn{3}{c}{Property 2}\\
%    \cline{2-7}
%    N& $M_1$ & $M_2$ & $M_3$ & $M_1$ & $M_2$ & $M_3$ \\
%    \cline{2-7}
%    %3&  & & & \\
    %4&  & & & \\
%    10& 0.070 & 0.041 & 0.040 & 0.085 & 0.346 & 0.039\\
%    20& 0.149 & 0.079 & 0.093 & 0.179 & 0.610 & 0.089\\
%    30& 0.212 & 0.098 & 0.139 & 0.254 &  & 0.133 \\
%    \cline{2-7}
%    \end{tabular}
%    \caption{\prism{} Results for Properties 1 \& 2 (5 bins); $M_1$: without run-time guard; $M_2$: with run-time guard; $M_3$: with run-time guard hard-coded to always pass}
    %\label{tab:prism_results}
%\end{table}






%\begin{table}[ht!]
%    \centering
    %\caption{Results for \prism{} Analysis (to be replaced with a graph)}  
%    \begin{tabular}{c|c||c|}
%    \multicolumn{1}{c}{}&\multicolumn{1}{c}{Property 3}&\multicolumn{1}{c}{Property 4}\\
%    \cline{2-3}
%    N& $M_2$ &  $M_2$ \\
%    \cline{2-3}
%    3& 0.44113550368388427 &  0.0547482360091121  \\
%    4& 0.5303800960048171  &  0.12838330391338953  \\
%    10& 0.7757822761375492 &  0.5842720053022902  \\
%    20& 0.8424710171917555 &  0.949333117789111 \\
%    30& 0.8481824509190194 & 0.9954975468019078\\
%    \cline{2-3}
%    \end{tabular}
%    \caption{\prism{} Results for Properties 3 \& 4 (to be replaced with a graph)}
%    \label{tab:prism_results}
%\end{table}



\paragraph{Results for Confidence Interval Analysis.} 
%-Run \prism{} analyses + confidence analysis \\
%- Show the scaling trend of confidence analysis as number of steps is increased.
Results for the confidence interval analysis are shown in Figures~\ref{fig:CI_taxinet}. The probabilities for the $\vcte$ failure and $\vhe$ failure are presented in Figure~\ref{fig:ci_p2} and in Figure~\ref{fig:ci_p1} for the confidence levels from $95\%$ up to $99\%$.
%\corina{to expand}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.475\textwidth}
         \centering         \includegraphics[width=\textwidth]{taxinet_plots/fact/taxinet_prop1.pdf}
         \caption{Confidence intervals for the property $P=? [ F (\vcte=-1)]$}
         \label{fig:ci_p2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.475\textwidth}
         \centering
        \includegraphics[width=\textwidth]{taxinet_plots/fact/taxinet_prop2.pdf}
         \caption{Confidence intervals for the property $P=? [ F (\vhe=-1)]$}
         \label{fig:ci_p1}
     \end{subfigure}
        \caption{Confidence interval results without run-time guard for 3-bins model}
        \label{fig:CI_taxinet}
\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.475\textwidth}
         \centering
         \includegraphics[width=\textwidth]{taxinet_plots/fact/taxinet_vc_prop1.pdf}
         \caption{Confidence intervals for the property $P=? [ F (\vcte=-1)]$}
         \label{fig:ci_vc_p1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.475\textwidth}
         \centering
         \includegraphics[width=\textwidth]{taxinet_plots/fact/taxinet_vc_prop2.pdf}
         \caption{Confidence intervals for the property $P=? [ F (\vhe=-1)]$}
         \label{fig:ci_vc_p2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{taxinet_plots/fact/taxinet_vc_prop3.pdf}
         \caption{Confidence intervals for the property $P=? [ F (v=0)]$}
        \label{fig:ci_vc_p3}
     \end{subfigure}
        \caption{Confidence interval results with run-time guard for 3-bins model}
        \label{fig:CI_taxinet_vc}
\end{figure}




\paragraph{Results of \prism{} and Confidence Interval Analysis (with Run-time Guard).}

\textcolor{red}{TODO: describe the experiments, bottleneck and refer to fPMC \cite{Fang22CGA}}


%\subsection{Line-following Robot}
%\label{sec:eval_line}
%-Set-up closed-loop experiment using simulator\\
%-TODO:Train perception model: (i) Generate data for training, (ii) Train model using Gloro training + calibration\\
%-Run end-to-end experiment on simulator + if time permits, physical experiment
%-Run \prism{} analyses + confidence analysis \\
%- Show the scaling trend of confidence analysis as number of steps is increased\\
%-Show effect on probability of abstention as the verification condition is varied (confidence thresholds vs robustness vs both)

\subsection{Discussion}
Our experiments highlight the potential of our approach to provide useful insights regarding the safety of an autonomous systems employing  complex image-based models for perception. 

- Highlight the compositional nature of the analysis; can replace taxinet with line-following net without any major change to the analysis + internals of networks, classifier vs regressor are irrelevant due to the abstraction

\corina{to be compressed; maybe move some of this discussion to Section 4.1?}
The \prism{} results point out that the TaxiNet system is more vulnerable to failure due to the plane going of the runway/taxiway than the plane turning more than a certain threshold. The highest probability of violating property 1 is 0.75 compared to violation of property 2 (0.12). While it is intuitive that the probability of failure increases with the length of the pathway, we can also observe that the rate of increase is much higher for property 1, while the system is more robust to property 2 as the length of the pathway increases. It is interesting to note that when we consider the classification accuracy of the Boeing model stand-alone, it performs better on the $\vcte$ prediction than the $\vhe$ prediction. However, the closed-loop system analysis highlights that the misclassification of $\vcte$ leads to the property violation more frequently than mis-classification wrt. $\vhe$.%in comparison with state-of-the-art[CITE STANFORD , UIUC, ALUR ].

The results also help highlight the benefit provided by the run-time guards. The rules not only helped improve the model behavior offline \ravi{what does offline mean here}, the closed-loop analysis shows that run-time guards lead to improvement in the safety of the overall system. The probabilities of failure decrease by an average of 68\% for property 1 and 81\% for property 2, with the system being almost 100\% robust (probability of failure close to 0) for property 2. It is interesting to note that the effectiveness of the guards become more pronounced as the length of the pathway increases. The probability of failure for N = 30 for property 1 is 0.138 which is 82\% lesser than without the guards, similarly for property 2 the decrease is 89\%. Note that we rejected only 17\% of all the inputs using the runtime guards.  

These results are produced almost instantaneously even for the largest value of N, which highlights the scalability of our technique. 
%{\bf not sure if we can quantitatively compare times with STANFORD, UIUC, ALUR }
It is important to note however that the soundness of these results is impacted by the size and the distribution of the dataset used to calculate the transition probabilities of the perception subsystem. The confidence interval analysis serves to add confidence in the computed probabilities. For instance, for N=4 in the absence of runtime guards, we can say with 99\% confidence that the probabilities of failure for property 2 would lie within [0.005,0.05] and for property 1 within [0.055,0.24]. Similarly, we can confirm that the system is robust wrt. property 2 because the probability of failure (0.003 for N=3) will only vary between [0,0.013] with 99\% confidence. We can also learn that higher values of N have higher variability in the probabilities of failure for a given confidence level.
%-Demonstrate scalability of the approach (compared to the scalability of symbolic techniques that do not abstract the visual data generation and perception components, for instance, Stanford work, Alur's paper or ones using deterministic abstactions like UIUC paper)\\
%- Demonstrate the positive effect of using run-time checks\\

The soundness of the abstraction of the perception module's behavior can be refined by including diverse inputs in the dataset.\ravi{Saying "soundness can be refined" does not make sense. Perhaps remove sentence} The inputs we used in our experiment does include images with shadows, skid marks on the pathway and images at night and day time. However, inclusion of more images with perturbations to semantic features such as contrast, brightness so on would improve the reliability of the results of our safety analysis. Our framework also accommodates composition of different scenarios which may require different controller actions. For instance, we could encode different DTMC models for moving in straight-line on the pathway vs making turns on the pathway, and compose the results.
We leave these for future work.

\corina{add statistics: time/memory consumed; mention computer configuration}

\corina{comment on actual results; error rates are pretty high; say the quality of the model is not great; also the controller and dynamics are toy models could be improved in the future; but our case study already highlights the benefits of the proposed approach: scalability of prism analysis, use of run time guards to improve precision, confidence analysis to provide guarantees}






==> section_related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Autonomous systems with learned components.}
analysis post controller synthesis; analysis and synthesis in a loop; safe reinforcement learning (i.e. reward shaping guided by logical safety specs)

\paragraph{Individual neural networks.}
Describe common specs and analysis techniques. These analyses are unable to provide system-level safety guarantees 


mention our previous case study paper

also works based on simulation/falsification (sanjit seshia's work)

%% moved from introduction
While formal proofs of closed-loop safety are feasible for systems with low-dimensional sensor readings ~\cite{santa2022nnlander,ivanov2021compositional,ivanov2019verisig,ivanov2020verifying,ivanov2021verisig}, these proofs become intractable when systems use rich sensors producing high-dimensional observations. 

First, not only is the generative process $g$ difficult to model mathematically~\cite{santa2022nnlander}, but also it depends on external environmental inputs $E$ that are difficult to account for. Second, even if one manages to construct a mathematical model of $g$,  the combined complexity of $g$ and the neural networks used for perception makes current closed-loop analysis algorithms too expensive.   Prior works have tried to address the modeling and scalability challenges by constructing simple, deterministic abstractions of the composition $p\circ g$ of the generator and the perception components~\cite{hsieh2022verifying,katz2022verification}.  %To ensure soundness of the analysis, these abstractions need to be over-approximate but this leads to an accumulation of approximation error as safety is verified over longer horizons. Consequently, existing techniques either forego any soundness guarantees about their abstractions~\cite{katz2022verification,santa2022nnlander} or  provide a probabilistic guarantees of soundness for the used abstraction~\cite{hsieh2022verifying}; however these are not probabilistic guarantees over teh safety of the system.
To deal with the environmental inputs, these abstract functions are made non-deterministic (i.e., of type $S \to 2^S$) encoding the fact that a single underlying system state can lead to multiple different sensor readings depending on the environmental inputs, and therefore, a set of possible perception outcomes.
However, these abstractions either lack soundness proofs~\cite{katz2022verification} or come with only probabilistic soundness guarantees~\cite{hsieh2022verifying} which however do not translate into probabilistic guarantees over the safety of the system.
An alternate approach for scaling closed-loop safety proofs is to construct inductive invariants in the form of barrier functions~\cite{alur2011formal,dawson2022learning,dawson2022safe,tong2022enforcing}. One only needs to prove that, over a single step of the system dynamics, the invariant is inductive and it implies safety. But constructing these invariants can be intractable in high-dimensional settings.


==> section_verification.tex <==
\section{Compositional Verification}
\label{sec:verif}

\subsection{Verification with Confidence Intervals}
\label{sec:verif_conf}
- Describe the FACT approach by Calinescu et al. and how we apply it to our setting

\subsection{Composing Proofs}
\label{sec:verif_compose}
- Describe how we compose the proofs obtained via FACT for each segment of the track into a proof for the entire track


==> tables/confusion_3bin_no_vc.tex <==
\begin{table*}[ht]
%\begin{scriptsize}
\resizebox{\textwidth}{!}{
\begin{tabular}
{|c|c|c|c|c|c|}\hline
{\textbf{Accuracy}}&\textbf{Grd Truth Label}&\textbf{Tot \# inputs}&\textbf{Actual Label}&\textbf{\# inputs}&\textbf{Trans Prob} \\\hline
\multirow{9}{*}{\textbf{CTE (78.67\%)}}&\multirow{3}{*}{1}&\multirow{3}{*}{1732}&1&552&0.319\\\cline{4-6}
&&&0&1180&0.681\\\cline{4-6}
&&&2&0&0.0\\\cline{2-6}
&\multirow{3}{*}{0}&\multirow{3}{*}{7054}&1&17&0.002\\\cline{4-6}
&&&0&6789&0.962\\\cline{4-6}
&&&2&248&0.036\\\cline{2-6}
&\multirow{3}{*}{2}&\multirow{3}{*}{2322}&1&0&0.0\\\cline{4-6}
&&&0&924&0.398\\\cline{4-6}
&&&2&1398&0.602\\\hline
%
\multirow{9}{*}{\textbf{HE (69.99\%)}}&\multirow{3}{*}{1}&\multirow{3}{*}{2101}&1&2010&0.957\\\cline{4-6}
&&&0&91&0.043\\\cline{4-6}
&&&2&0&0.0\\\cline{2-6}
&\multirow{3}{*}{0}&\multirow{3}{*}{7035}&1&2139&0.304\\\cline{4-6}
&&&0&4748&0.675\\\cline{4-6}
&&&2&148&0.021\\\cline{2-6}
&\multirow{3}{*}{2}&\multirow{3}{*}{1972}&1&211&0.107\\\cline{4-6}
&&&0&744&0.377\\\cline{4-6}
&&&2&1017&0.516\\\hline
\end{tabular}}
%\end{scriptsize}
\caption{Results for all inputs. Total of 11108 inputs. The regression model MAE for $\vcte$ is 1.185 and for $\vhe$ is 7.860.}
\label{tab:trans_prob}
\end{table*}

==> tables/fact_3bin_perf.tex <==
\begin{table}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{lllcll|lll|}
\cline{7-9}
&                         &                                           & \multicolumn{1}{l}{}                                                                            &                                                           &                                    & \multicolumn{3}{l|}{Time (s) for computing CI levels}                                     \\ \hline
\multicolumn{1}{|c|}{Model}                          & \multicolumn{1}{l|}{N}  & \multicolumn{1}{l|}{Property}             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Model Size\\ (States, transitions)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}PMC result\\ String size, time(s)\end{tabular}} & \multicolumn{1}{l|}{95}       & \multicolumn{1}{l|}{97}           & 99                    \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_fact}     & \multicolumn{1}{l|}{3}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{c|}{217,331}                                                                    & \multicolumn{1}{l|}{36}                                   & 1.476                              & \multicolumn{1}{l|}{2.845}    & \multicolumn{1}{l|}{2.564}        & 2.587                 \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_fact}     & \multicolumn{1}{l|}{4}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{c|}{422, 650}                                                                   & \multicolumn{1}{l|}{262}                                  & 1.456                              & \multicolumn{1}{l|}{4.96}     & \multicolumn{1}{l|}{2.88}         & 2.92                  \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_fact}     & \multicolumn{1}{l|}{5}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{c|}{703,1102}                                                                   & \multicolumn{1}{l|}{3496}                                 & 1.448                              & \multicolumn{1}{l|}{4.79}     & \multicolumn{1}{l|}{6.48}         & 21.09                 \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_fact}     & \multicolumn{1}{l|}{6}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{c|}{984,1554}                                                                   & \multicolumn{1}{l|}{19832}                                & 1.493                              & \multicolumn{1}{l|}{10.03}    & \multicolumn{1}{l|}{11.21}        & 45.68                 \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_fact}     & \multicolumn{1}{l|}{7}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{c|}{1265,2006}                                                                  & \multicolumn{1}{l|}{76557}                                & 1.478                              & \multicolumn{1}{l|}{52.8}     & \multicolumn{1}{l|}{65.5}         & 338.7                 \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_fact}     & \multicolumn{1}{l|}{8}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{c|}{1546, 2458}                                                                 & \multicolumn{1}{l|}{275372}                               & 2.117                              & \multicolumn{1}{l|}{843.25}   & \multicolumn{1}{l|}{938.69}       & 5334.48               \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_fact}     & \multicolumn{1}{l|}{9}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{c|}{1827,2910}                                                                  & \multicolumn{1}{l|}{893783}                               & 3.729                              & \multicolumn{1}{c|}{6227.988} & \multicolumn{1}{l|}{7442.884(2h)} & 4 hours-still running \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_fact}     & \multicolumn{1}{l|}{10} & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{l|}{}                                                                           & \multicolumn{1}{l|}{no PMC}                               &                                    & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}             &                       \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_fact}     & \multicolumn{1}{l|}{3}  & \multicolumn{1}{l|}{P=? {[} F cte=-1 {]}} & \multicolumn{1}{c|}{217,331}                                                                    & \multicolumn{1}{l|}{151}                                  & 1.709                              & \multicolumn{1}{l|}{3.435}    & \multicolumn{1}{l|}{3.521}        & 3.264                 \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_fact}     & \multicolumn{1}{l|}{4}  & \multicolumn{1}{l|}{P=? {[} F cte=-1 {]}} & \multicolumn{1}{c|}{422,650}                                                                    & \multicolumn{1}{l|}{1453}                                 & 1.571                              & \multicolumn{1}{l|}{12.462}   & \multicolumn{1}{l|}{13.976}       & 36.378                \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_fact}     & \multicolumn{1}{l|}{5}  & \multicolumn{1}{l|}{P=? {[} F cte=-1 {]}} & \multicolumn{1}{c|}{703,1102}                                                                   & \multicolumn{1}{l|}{6604}                                 & 1.483                              & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{timeout}      &                       \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing5bins\_fact}     & \multicolumn{1}{l|}{4}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{c|}{854,1440}                                                                   & \multicolumn{1}{l|}{1400}                                 & 1.725                              & \multicolumn{1}{l|}{7.728}    & \multicolumn{1}{l|}{5.779}        &                       \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing5bins\_fact}     & \multicolumn{1}{l|}{5}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{c|}{1554,2661}                                                                  & \multicolumn{1}{l|}{12859}                                & 1.816                              & \multicolumn{1}{l|}{1081}     & \multicolumn{1}{l|}{}             &                       \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_vc\_fact} & \multicolumn{1}{l|}{3}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{c|}{269,429}                                                                    & \multicolumn{1}{l|}{153}                                  & 1.705                              & \multicolumn{1}{l|}{7.753}    & \multicolumn{1}{l|}{2.433}        & 3.693                 \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_vc\_fact} & \multicolumn{1}{l|}{4}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{c|}{531,839}                                                                    & \multicolumn{1}{l|}{1040}                                 & 1.462                              & \multicolumn{1}{l|}{3.461}    & \multicolumn{1}{l|}{3.161}        & 2.933                 \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing3bins\_vc\_fact} & \multicolumn{1}{l|}{5}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{c|}{886,1449}                                                                   & \multicolumn{1}{l|}{12266}                                & 2.089                              & \multicolumn{1}{l|}{18.46}    & \multicolumn{1}{l|}{24.383}       & 30.69                 \\ \hline
\multicolumn{1}{|l|}{taxinet\_Boeing5bins\_vc\_fact} & \multicolumn{1}{l|}{3}  & \multicolumn{1}{l|}{P=? {[} F he=-1 {]}}  & \multicolumn{1}{l|}{}                                                                           & \multicolumn{1}{l|}{}                                     &                                    & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}             &                       \\ \hline
\end{tabular}
}
\caption{\fact{} performance statistics. Experiments are run on a Windows OS machine with 11th Gen Intel(R) Core(TM) i7 processor and 64GB RAM.}
\end{table}

==> tables/old_prism_results.tex <==
%\begin{table}[ht!]
%    \centering
    %\caption{Results for \prism{} Analysis (to be replaced with a graph)}
   
%    \begin{tabular}{c|c|c|c||c|c|c|}
%    \multicolumn{1}{c}{}&\multicolumn{3}{c}{Property 1}&\multicolumn{3}{c}{Property 2}\\
%    \cline{2-7}
%    N& $M_1$ & $M_2$ & $M_3$ & $M_1$ & $M_2$ & $M_3$ \\
%    \cline{2-7}
    %3&  & & & \\
    %4&  & & & \\
%    10& 0.391 & 0.208 & 0.302 & 0.060 & 0.290 & 0.027\\
%    20& 0.632 & 0.335 & 0.538 & 0.099 & 0.465 & 0.049\\
%    30& 0.749 & 0.385 & 0.683 & 0.118 & 0.535 & 0.063\\
%    \cline{2-7}
%    \end{tabular}
%    \caption{\prism{} Results for Properties 1 \& 2 (3 bins); $M_1$: without run-time guard; $M_2$: with run-time guard; $M_3$: with run-time guard hard-coded to always pass}
    %\label{tab:prism_results}
%\end{table}

%\begin{table}[ht!]
%    \centering
%    %\caption{Results for \prism{} Analysis (to be replaced with a graph)}
   
%    \begin{tabular}{c|c|c|c||c|c|c|}
%    \multicolumn{1}{c}{}&\multicolumn{3}{c}{Property 1}&\multicolumn{3}{c}{Property 2}\\
%    \cline{2-7}
%    N& $M_1$ & $M_2$ & $M_3$ & $M_1$ & $M_2$ & $M_3$ \\
%    \cline{2-7}
%    %3&  & & & \\
    %4&  & & & \\
%    10& 0.070 & 0.041 & 0.040 & 0.085 & 0.346 & 0.039\\
%    20& 0.149 & 0.079 & 0.093 & 0.179 & 0.610 & 0.089\\
%    30& 0.212 & 0.098 & 0.139 & 0.254 &  & 0.133 \\
%    \cline{2-7}
%    \end{tabular}
%    \caption{\prism{} Results for Properties 1 \& 2 (5 bins); $M_1$: without run-time guard; $M_2$: with run-time guard; $M_3$: with run-time guard hard-coded to always pass}
    %\label{tab:prism_results}
%\end{table}

%\begin{table}[ht!]
%    \centering
    %\caption{Results for \prism{} Analysis (to be replaced with a graph)}  
%    \begin{tabular}{c|c||c|}
%    \multicolumn{1}{c}{}&\multicolumn{1}{c}{Property 3}&\multicolumn{1}{c}{Property 4}\\
%    \cline{2-3}
%    N& $M_2$ &  $M_2$ \\
%    \cline{2-3}
%    3& 0.44113550368388427 &  0.0547482360091121  \\
%    4& 0.5303800960048171  &  0.12838330391338953  \\
%    10& 0.7757822761375492 &  0.5842720053022902  \\
%    20& 0.8424710171917555 &  0.949333117789111 \\
%    30& 0.8481824509190194 & 0.9954975468019078\\
%    \cline{2-3}
%    \end{tabular}
%    \caption{\prism{} Results for Properties 3 \& 4 (to be replaced with a graph)}
%    \label{tab:prism_results}
%\end{table}
